Defining and Characterizing Reward Hacking

We provide the first formal definition of reward hacking, a phenomenon where optimizing an imperfect proxy reward function leads to poor performance according to the true reward function. We say that a proxy is unhackable if increasing the expected proxy return can never decrease the expected true return. Intuitively, it might be possible to create an unhackable proxy by leaving some terms out of the reward function (making it "narrower") or overlooking fine-grained distinctions between roughly equivalent outcomes, but we show this is usually not the case. A key insight is that the linearity of reward (in state-action visit counts) makes unhackability a very strong condition. In particular, for the set of all stochastic policies, two reward functions can only be unhackable if one of them is constant. We thus turn our attention to deterministic policies and finite sets of stochastic policies, where non-trivial unhackable pairs always exist, and establish necessary and sufficient conditions for the existence of simplifications, an important special case of unhackability. Our results reveal a tension between using reward functions to specify narrow tasks and aligning AI systems with human values.

==> backup_thm_1 <==
\begin{theorem} \label{thm:open-set} % TODO: informal
In any $MDP \setminus \mathcal{R}$, if $\hat{\Pi}$ contains an open set, then any pair of reward functions that are ungameable and non-trivial on $\hat{\Pi}$ are equivalent on $\hat{\Pi}$.
\end{theorem}
\begin{proof}

% Let $R'_1$ and $R'_2$ be arbitrary ungameable and non-trivial reward functions, and define normalized versions $R_1 = \frac{R'_1}{||R'_1||_2}$ and $R_2 = \frac{R'_2}{||R'_2||_2}$.  
% Note that $R_1$ is equivalent to $R'_1$, and $R_2$ is equivalent to $R'_2$.
Let $\mathcal{R}_1$ and $\mathcal{R}_2$ be any two ungameable and non-trivial reward functions.
We will show that, for any $\pi, \pi' \in \hat{\Pi}$, we have $J_1(\pi) = J_1(\pi') \implies J_2(\pi) = J_2(\pi')$, and thus, by symmetry, $J_1(\pi) = J_1(\pi') \iff J_2(\pi) = J_2(\pi')$.
Since $\mathcal{R}_1$ and $\mathcal{R}_2$ are ungameable, this means they have the exact same policy order, i.e.\ they are equivalent. {\color{red} TODO: fix preceding sentence}

Choose two arbitrary $\pi, \pi' \in \hat{\Pi}$ with $J_1(\pi) = J_1(\pi')$ and let $f \doteq \mathcal{F}(\pi), f' \doteq \mathcal{F}(\pi')$.
The proof has 3 steps:% are as follows:
\begin{enumerate}
    \item We find analogues for $f$ and $f'$, $\tilde{f}$ and $\tilde{f'}$, within the same open ball.
    \item We show that the level sets of $\mathcal{R}_1$ and $\mathcal{R}_2$ at $\tilde{f}$ must be equal to prevent neighbors of $\tilde{f}$ from making $\mathcal{R}_1$ and $\mathcal{R}_2$ gameable.
    \item We use linearity to show that this implies that $J_2(\pi) = J_2(\pi')$.
    %\item Since equivalence is transitive, $R'_1$ and $R'_2$ are also equivalent, completing the proof.
\end{enumerate}
% The proof proceeds by finding an analogue for $f$, soit $\hat{f}$, that is contained within an open set.
% Then, (ii) we show that the level sets of $R_1$ and $R_2$ must be equal to prevent neighbors of $\hat{f}$ making $R_1$ and $R_2$ gameable.
% Finally, this allows us to show that these level sets are equal at $\pi$ as well, and so $R_1$ and $R_2$ are equivalent.

\textbf{Step 1:}
First, because $\hat{\Pi}$ contains an open set, we can find some $\hat{\pi}$ such that $\hat{f} \doteq \mathcal{F}(\hat{\pi})$ is the center of an open ball.
Then, for small enough $\delta$, we have $\tilde{f} \doteq \hat{f} + \delta f$ and $\tilde{f'} \doteq \hat{f} + \delta f'$ are both inside this open ball.

\textbf{Step 2:}
%For any policy $\dot{\pi}$, define 
Let $\tilde{\pi}$ be the policy with visit counts $\tilde{f}$.
Consider the level sets $H_1, H_2$, defined as those policies with the same value of $\tilde{\pi}$ according to $\mathcal{R}_1$ or $\mathcal{R}_2$, respectively.
Note that if we consider reward functions as vectors in $\mathbb{R}^{|S||A|}$, then non-trivial reward functions have corresponding tangent planes, and these level sets are given by the intersection of these tangent planes with our policy set $\hat{\Pi}$.
% Now, unless $H_1 = H_2$, then we can move in $H_1$ in a direction that increases reward according to $R_2$, and vice versa; i.e.\ we can find $f_1 \in H_1$, $f_2 \in H_2$ such that $R_1(f_1) > R_1(f) > $ 
%Now, suppose $H_1 \neq H_2$ consider the reward function $R_{12} \doteq \frac{R_1 - R_2}{2}$. 
%It's level set $H_{12}(\tilde{\pi})$ contains a point from within the open ball around $\tilde{f}$, soit $f_{12}$, and we have
Now, if $H_1 \neq H_2$ we can find a point from within the open ball around $\tilde{f}$, that is above $H_1$ and below $H_2$, whose visit counts are realized by policy $\pi_{12}$.  This yielding $J_1(\pi_{12}) > J_1(\tilde{\pi})$ and $J_2(\pi_{12}) < J_2(\tilde{\pi})$, a contradiction.
Thus $H_1 = H_2$.

\textbf{Step 3:}
Since $H_1 = H_2$, we also have (considering $J \doteq \langle \mathcal{R}, \cdot \rangle$ as a function of visit counts) $J_2(\tilde{f}) = J_2(\tilde{f'})$. 
Expanding, we have: $J_2(\hat{f} + \delta f) = J_2(\hat{f} + \delta f')$, and thus by linearity we have $J_2(f) = J_2(f')$, i.e.\ 
$J_2(\pi) = J_2(\pi')$.
\end{proof}
